SALAD: Source-free Active Label-Agnostic Domain Adaptation for Classification, Segmentation and Detection

We present a novel method, SALAD, for the challenging vision task of adapting a pre-trained "source" domain network to a "target" domain, with a small budget for annotation in the "target" domain and a shift in the label space. Further, the task assumes that the source data is not available for adaptation, due to privacy concerns or otherwise. We postulate that such systems need to jointly optimize the dual task of (i) selecting fixed number of samples from the target domain for annotation and (ii) transfer of knowledge from the pre-trained network to the target domain. To do this, SALAD consists of a novel Guided Attention Transfer Network (GATN) and an active learning function, HAL. The GATN enables feature distillation from pre-trained network to the target network, complemented with the target samples mined by HAL using transfer-ability and uncertainty criteria. SALAD has three key benefits: (i) it is task-agnostic, and can be applied across various visual tasks such as classification, segmentation and detection; (ii) it can handle shifts in output label space from the pre-trained source network to the target domain; (iii) it does not require access to source data for adaptation. We conduct extensive experiments across 3 visual tasks, viz. digits classification (MNIST, SVHN, VISDA), synthetic (GTA5) to real (CityScapes) image segmentation, and document layout detection (PubLayNet to DSSE). We show that our source-free approach, SALAD, results in an improvement of 0.5%-31.3%(across datasets and tasks) over prior adaptation methods that assume access to large amounts of annotated source data for adaptation.

==> Tables/datasets.tex <==
\begin{table}
% \footnotesize
\centering
\scriptsize
% \begin{center}
% \resizebox{0.6\columnwidth}{!}
{
\begin{tabular}{c c c c c}
\toprule
Source & Target & Task & Label Shift & Eval. \\ 
\toprule
MNIST \cite{deng2012mnist} & SVHN \cite{sermanet2012convolutional} & Classification & No & Accuracy\\
SVHN \cite{sermanet2012convolutional}  & MNIST \cite{deng2012mnist} & Classification & No & Acc.\\
MNIST \cite{deng2012mnist} & SVHN \cite{sermanet2012convolutional}  & Classification & Yes (2 cases) & Acc.\\
%VISDA17 Syn \cite{peng2017visda} & VISDA17 Real \cite{peng2017visda} & Classification & No & Acc.\\
GTA5 \cite{richter2016playing} & CityScapes \cite{cordts2016cityscapes} & Segmentation & No & Acc., IoU\\
Publaynet \cite{zhong2019publaynet} & DSSE \cite{yang2017learning} & Document Layout Detection & Yes & mAP\\
\bottomrule
\end{tabular}
}
%The final column contains the evaluation metrics. 
% While most prior methods are customized to tasks/ output label space configuration, \model~ can be applied across various visual tasks and is label space agnostic.
\caption{\small{\textbf{Tasks and Datasets:} The source and target datasets are listed in the first two columns. %The third column lists the corresponding tasks, and 
The fourth column indicates whether there is a shift in label space while adapting from the source to the target domain.}}
\label{tab:datasets}
%\vspace{-20pt}
% \end{center}
\end{table}

